SoK: The Gap Between Data Rights Ideals and Reality

As information economies burgeon, they unlock innovation and economic wealth while posing novel threats to civil liberties and altering power dynamics between individuals, companies, and governments. Legislatures have reacted with privacy laws designed to empower individuals over their data. These laws typically create rights for "data subjects" (individuals) to make requests of data collectors (companies and governments). The European Union General Data Protection Regulation (GDPR) exemplifies this, granting extensive data rights to data subjects, a model embraced globally. However, the question remains: do these rights-based privacy laws effectively empower individuals over their data? This paper scrutinizes these approaches by reviewing 201 interdisciplinary empirical studies, news articles, and blog posts. We pinpoint 15 key questions concerning the efficacy of rights allocations. The literature often presents conflicting results regarding the effectiveness of rights-based frameworks, but it generally emphasizes their limitations. We offer recommendations to policymakers and Computer Science (CS) groups committed to these frameworks, and suggest alternative privacy regulation approaches.

==> new_papers.tex <==
Human-GDPR Interaction: Practical Experiences of Accessing Personal Data
https://dl.acm.org/doi/abs/10.1145/3491102.3501947

Economic Research on Privacy Regulation: Lessons from the GDPR and Beyond
https://www.nber.org/papers/w30705 --> Can we add this to the section C8?


